Low-Resource Cross-Lingual Summarization through Few-Shot Learning with Large Language Models

Cross-lingual summarization (XLS) aims to generate a summary in a target language different from the source language document. While large language models (LLMs) have shown promising zero-shot XLS performance, their few-shot capabilities on this task remain unexplored, especially for low-resource languages with limited parallel data. In this paper, we investigate the few-shot XLS performance of various models, including Mistral-7B-Instruct-v0.2, GPT-3.5, and GPT-4. Our experiments demonstrate that few-shot learning significantly improves the XLS performance of LLMs, particularly GPT-3.5 and GPT-4, in low-resource settings. However, the open-source model Mistral-7B-Instruct-v0.2 struggles to adapt effectively to the XLS task with limited examples. Our findings highlight the potential of few-shot learning for improving XLS performance and the need for further research in designing LLM architectures and pre-training objectives tailored for this task. We provide a future work direction to explore more effective few-shot learning strategies and to investigate the transfer learning capabilities of LLMs for cross-lingual summarization.

==> Tables/Table1.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{table*}
{\LARGE
  \centering
  \setlength{\tabcolsep}{8pt}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{lSSSSSSSSSSSSSSSSSSS|SSSSSSSSSSSSSSSSSSS}
        \toprule[3pt]
        \multicolumn{2}{c}{} & \multicolumn{36}{c}{LangPair} \\
        \cmidrule(rl){3-38}
        \multicolumn{2}{c}{Models} & \multicolumn{3}{c}{Th-En}   & \multicolumn{3}{c}{Gu-En}  & \multicolumn{3}{c}{Mr-En} & \multicolumn{3}{c}{Pa-En}  & \multicolumn{3}{c}{Bu-En} & \multicolumn{3}{c|}{Si-En} & \multicolumn{3}{c}{En-Th} & \multicolumn{3}{c}{En-Gu} & \multicolumn{3}{c}{En-Mr}  & \multicolumn{3}{c}{En-Pa} & \multicolumn{3}{c}{En-Bu} & \multicolumn{3}{c}{En-Si}\\
        \cmidrule(rl){3-5} \cmidrule(rl){6-8} \cmidrule(rl){9-11} \cmidrule(rl){12-14} \cmidrule(rl){15-17} \cmidrule(rl){18-20} \cmidrule(rl){21-23} \cmidrule(rl){24-26} \cmidrule(rl){27-29} \cmidrule(rl){30-32} \cmidrule(rl){33-35} \cmidrule(rl){36-38} 
          {}                & {}           & {R1}           & {R2}           & {RL}           & {R1}           & {R2}           & {RL}           & {R1}           & {R2}           & {RL}           & {R1}           & {R2}           & {RL}          & {R1}           & {R2}           & {RL}      
        & {R1}           & {R2}           & {RL}          & {R1}           & {R2}           & {RL}      
        & {R1}           & {R2}           & {RL}          & {R1}           & {R2}           & {RL}      
        & {R1}           & {R2}           & {RL}          & {R1}           & {R2}           & {RL}      
        & {R1}           & {R2}           & {RL}\\
        \cmidrule[3pt](rl){1-38}
          \multicolumn{2}{c}{MT5}      & {29.16}             & {9.79}         & {22.63}          & {24.28}         & {6.4}     & {19.12}          & {25.87}         & {7.28}          & {20.14}         & {30.86}  & {10.27}      & {24.78}             & {28.44}         & {7.5}         & {22.07}             & {28.94}         & {8.17}       & {22.53}             & {4.59}         & {0.94}             & {4.4}         & {10.14}             & {1.19}         & {9.37}        & {9.38}             & {1.22}         & {8.94}          & {20.12}             & {4.62}         & {17.55}          & {4.85}             & {0.55}         & {4.72}           & {5.62}             & {0.39}         & {5.13} \\
          \cmidrule(rl){1-38}
         {}    &{Zero-shot}       & {14.69}             & {3.84}         & {10.32}          & {12.69}         & {2.8}     & {9.2}          & {13.83}         & {3.04}          & {9.96}         & {14.98}  & {3.78}      & {10.94}             & {13.2}         & {2.21}         & {10.19}             & {13.08}         & {2.11}       & {9.91}             & {4.78}         & {1.48}             & {4.53}         & {1.4}             & {0.0}         & {1.4}        & {2.05}             & {0.0}         & {2.05}          & {0.0}             & {0.0}         & {0.0}          & {1.7}             & {0.26}         & {1.7}           & {1.22}             & {0.0}         & {1.22} \\
         \cmidrule[0.01pt](rl){2-2}
          \multicolumn{1}{c}{GPT-3.5} &{One-shot}       & {15.18}             & {3.95}         & {10.99}          & {13.0}         & {3.12}     & {9.25}          & {14.91}         & {3.73}          & {10.79}         & {14.62}  & {3.93}      & {10.8}             & {15.8}         & {2.43}         & {11.91}             & {13.39}         & {2.34}       & {10.11}             & {4.5}         & {0.82}             & {4.45}         & {1.6}             & {0.0}         & {1.6}        & {1.02}             & {0.13}         & {1.02}          & {0.0}             & {0.0}         & {0.0}          & {0.58}             & {0.0}         & {1.55}           & {1.72}             & {1.72}         & {1.72} \\
          \cmidrule[0.01pt](rl){2-2}
          {}           &{Two-shot}       & {16.56}             & {4.59}         & {11.6}          & {15.33}         & {3.57}     & {10.57}          & {16.52}         & {4.06}          & {11.96}         & {15.52}  & {3.96}      & {11.06}             & {16.48}         & {2.83}         & {12.39}             & {14.03}         & {2.47}       & {9.81}             & {5.29}         & {1.46}             & {5.2}         & {0.55}       & {0.0}         & {0.55}      & {0.88}         & {0.09}        & {0.88}             & {0.0}         & {0.0}          & {0.0}             & {1.55}         & {0.0}          & {1.55}             & {1.72}         & {1.72}           & {1.72}              \\
          \cmidrule(rl){1-38}
          {}    &{Zero-shot}       & {12.22}             & {3.39}         & {8.59}          & {10.96}         & {2.71}     & {7.63}          & {10.97}         & {2.84}          & {7.9}         & {12.1}  & {3.58}      & {8.55}             & {14.73}         & {3.77}         & {9.84}             & {13.92}         & {3.86}       & {9.45}             & {6.09}         & {1.42}             & {5.84}         & {1.5}             & {0.0}         & {1.5}        & {1.35}             & {0.0}         & {1.35}          & {0.0}             & {0.0}         & {0.0}          & {2.61}             & {0.9}         & {2.61}           & {3.34}             & {1.72}         & {3.34} \\
         \cmidrule[0.01pt](rl){2-2}
          \multicolumn{1}{c}{GPT-4} &{One-shot}       & {14.86}             & {4.12}         & {10.51}          & {13.88}         & {3.5}     & {9.27}          & {14.11}         & {3.52}          & {10.09}         & {13.65}  & {4.15}      & {9.49}             & {16.88}         & {4.48}         & {11.41}             & {15.03}         & {4.35}       & {10.27}             & {9.38}         & {2.25}             & {9.38}         & {1.22}             & {0.0}         & {1.22}        & {1.48}             & {0.1}         & {1.48}          & {0.0}             & {0.0}         & {0.0}          & {4.62}             & {0.17}         & {4.62}           & {4.36}             & {1.15}         & {4.36} \\
          \cmidrule[0.01pt](rl){2-2}
          {}           &{Two-shot}       & {17.67}             & {5.19}         & {12.67}          & {13.63}         & {3.49}     & {9.27}          & {14.97}         & {3.73}          & {10.38}         & {13.65}  & {4.15}      & {9.49}             & {17.38}         & {4.32}         & {11.73}             & {15.1}         & {4.15}       & {10.39}             & {8.64}         & {2.16}             & {8.39}         & {2.05}             & {0.0}         & {2.05}        & {1.31}             & {0.0}         & {1.31}          & {0.0}             & {0.0}         & {0.0}          & {2.02}             & {0.22}         & {2.02}           & {2.53}             & {1.15}         & {2.53} \\
          \cmidrule(rl){1-38}
          \multirow{3}{*}{\makecell{Mistral-7B-\\instruct-v0.2}}    &{Zero-shot}       & {8.91}             & {2.12}         & {6.42}          & {6.15}         & {0.68}     & {4.76}          & {7.63}         & {1.55}          & {5.76}         & {7.65}  & {1.62}      & {5.99}             & {7.59}         & {1.06}         & {5.68}             & {7.23}         & {0.99}       & {5.4}             &{4.33}         & {1.18}             & {4.33}         & {0.23}             & {0.0}         & {0.23}        & {2.37}             & {0.2}         & {2.37}          & {0.0}             & {0.0}         & {0.0}          & {2.64}             & {1.21}         & {2.64}           & {0.06}             & {0.0}         & {0.06} \\
         \cmidrule[0.01pt](rl){2-2}
         &{One-shot}       & {10.28}             & {2.51}         & {7.58}          & {7.27}         & {0.79}     & {5.46}          & {8.08}         & {1.42}          & {6.06}         & {7.41}  & {1.21}      & {5.82}             & {8.35}         & {0.91}         & {6.37}             & {8.43}         & {1.06}       & {6.08}             & {4.39}         & {1.33}             & {4.3}         & {0.51}             & {0.0}         & {0.51}        & {1.64}             & {0.08}         & {1.64}          & {0.0}             & {0.0}         & {0.0}          & {7.78}             & {1.55}         & {7.78}           & {0.74}             & {0.0}         & {0.74} \\
          \cmidrule[0.01pt](rl){2-2}
          &{Two-shot}       & {10.1}             & {2.37}         & {7.3}          & {6.31}         & {0.71}     & {4.81}          & {6.66}         & {0.57}          & {5.35}         & {8.96}  & {1.71}      & {6.77}             & {9.55}         & {1.07}         & {7.44}             & {8.21}         & {0.49}       & {6.58}             & {3.15}         & {0.38}             & {2.94}         & {0.51}             & {0.0}         & {0.51}        & {0.55}             & {0.0}         & {0.55}          & {0.0}             & {0.0}         & {0.0}          & {2.43}             & {0.01}         & {2.1}           & {0.42}             & {0.0}         & {0.42} \\
        \bottomrule[3pt]
    \end{tabular}
    }
    \caption{Comprehensive comparison of model performance metrics across various language pairs, including R1, R2, and Rouge-L scores. The language pairs are abbreviated as follows: Th-En (Thai to English), Gu-En (Gujarati to English), Mr-En (Marathi to English), Pa-En (Pashto to English), Bu-En (Burmese to English), Si-En (Sinhala to English), En-Th (English to Thai), En-Gu (English to Gujarati), En-Mr (English to Marathi), En-Pa (English to Pashto), En-Bu (English to Burmese), and En-Si (English to Sinhala).}
  \label{tab:grav4}
  \vspace{-5mm}
}
\end{table*}

==> subcode.tex <==
\[
\begin{array}{p{0.95\textwidth}}
\textbf{Please summarize the following text in \{target language\}} \\\\
\textbf{Example 1} \\
\text{Text:} \{Example1 source text\} \\
\text{Translated summary:} \{Example1 target summary\} \\\\
\textbf{Example 2} \\
\text{Text:} \{Example2 source text]\} \\
\text{Translated summary:} \{Example2 target summary\} \\\\
\textbf{Test Text} \\
\text{Text:} \{test source text\} \\
\text{Translated summary:} \\\\
\end{array}
\]



\begin{table*}[!t]
{\scriptsize
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.2}

\resizebox{2.05\columnwidth}{!}{

\begin{tabular}{p{16cm}}
\toprule
\textbf{Input Prompt} \\
\midrule
\begin{array}{p{0.95\textwidth}}
\textbf{Please summarize the following text in \{target language\}} \\\\
\textbf{Example 1} \\
\text{Text:} \{validation["text"][1]\} \\
\text{Translated summary:} \{validation["summary"][1]\} \\\\
\textbf{Example 2} \\
\text{Text:} \{validation["text"][2]\} \\
\text{Translated summary:} \{validation["summary"][2]\} \\\\
\textbf{Test Text} \\
\text{Text:} \{test["text"]\} \\
\text{Translated summary:} \\\\
\end{array} 
% Intimacy: \{\textcolor{blue}{intimacy}\}\\
A:\\
%Generate Example:\\
\bottomrule
\end{tabular}

}

\caption{Prompt used to generate sarcastic dialogue $D'$ in section~\ref{subsec:generate_dialog}. The words colored \textit{blue} respectively indicates $S$, $p_a$, and $p_b$, extracted from $D$.}
\label{tab:prompt}
}
%\vspace{-5mm}
\end{table*}
